FoldToken2: Learning compact, invariant and generative protein structure language

The equivalent nature of 3D coordinates has posed long term challenges in protein structure representation learning, alignment, and generation. Can we create a compact and invariant language that equivalently represents protein structures? Towards this goal, we propose FoldToken2 to transfer equivariant structures into discrete tokens, while maintaining the recoverability of the original structures. From FoldToken1 to FoldToken2, we improve three key components: (1) invariant structure encoder, (2) vector-quantized compressor, and (3) equivalent structure decoder. We evaluate FoldToken2 on the protein structure reconstruction task and show that it outperforms previous FoldToken1 by 20\% in TMScore and 81\% in RMSD. FoldToken2 probably be the first method that works well on both single-chain and multi-chain protein structures quantization. We believe that FoldToken2 will inspire further improvement in protein structure representation learning, structure alignment, and structure generation tasks.

==> tables/reconstruction2.tex <==
\begin{table}[h]
   \resizebox{1.0 \columnwidth}{!}{
   \begin{tabular}{llllllllllll} 
       \toprule
   \multirow{2}{*}{Group}         & \multicolumn{5}{c}{Config}                                                                                                                          & \multicolumn{3}{c}{TMScore}           & \multicolumn{3}{c}{RMSD}               \\
                                  & \multicolumn{1}{c}{\#Code} & \multicolumn{1}{c}{\#Enc} & \multicolumn{1}{c}{\#Dec} & \multicolumn{1}{c}{\#Hid} & \multicolumn{1}{c}{\#KNN} & \multicolumn{1}{c}{Avg} & Max  & Min  & \multicolumn{1}{c}{Avg} & Max   & Min  \\ \hline
   FoldToken V1     & 65536    &    &     &    &     & 0.74   & 0.96 & 0.44 & 3.09   & 18.09 & 0.48 \\ \hline
   \multirow{14}{*}{FoldToken V2} & 65536                           & 6                         & 8                         & 128                       & 30                            & 0.84                    & 0.95 & 0.61 & 1.63                    & 4.85  & 1.10 \\
   & \chl 65536                           & \chl 8                         & \chl 8                         & \chl  128                       & \chl 30                            & \chl 0.88                    & \chl 0.97 & \chl 0.68 & \chl 1.38                    & \chl 10.92  & \chl 0.95 \\
   & 65536                           & 10                        & 8                         & 128                       & 30                            & 0.86                    & 0.96 & 0.49 & 1.81                    & 17.56  & 0.58 \\
   & 65536                           & 12                        & 8                         & 128                       & 30                            & 0.36                    & 0.68 & 0.21 & 9.53                    & 27.33 & 2.77 \\
   & 65536                           & 6                         & 10                        & 128                       & 30                            & 0.82                    & 0.94 & 0.56 & 1.68                    & 11.89  & 1.29 \\
   & 65536                           & 6                         & 12                        & 128                       & 30                            & 0.77                    & 0.93 & 0.47 & 2.22                    & 7.67  & 1.36 \\
   & 65536                           & 6                         & 15                        & 128                       & 30                            & 0.71                    & 0.89 & 0.45 & 2.65                    & 11.46  & 1.95 \\
   & 65536                           & 6                         & 10                        & 256                       & 30                            & 0.28                    & 0.41 & 0.12 & 14.30                   & 59.28 & 6.27 \\
   & 65536                           & 6                         & 10                        & 128                       & 50                            & 0.78                    & 0.91 & 0.55 & 2.11                    & 7.28  & 1.45 \\
   & 1024                            & 6                         & 10                        & 128                       & 30                            & 0.71                    & 0.88 & 0.38 & 3.17                    & 15.21  & 1.29 \\
   & 512                             & 6                         & 10                        & 128                       & 30                            & 0.38                    & 0.67 & 0.19 & 9.01                    & 49.81 & 2.58 \\
   & 256                             & 6                         & 10                        & 128                       & 30                            & 0.43                    & 0.75 & 0.17 & 11.96                    & 27.52 & 5.20 \\
   & 32                              & 6                         & 10                        & 128                       & 30                            & 0.27                    & 0.41 & 0.17 & 11.96                   & 27.52 & 5.20 \\
   & 16                              & 6                         & 10                        & 128                       & 30                            & 0.27                    & 0.43 & 0.13 & 14.09                   & 59.69 & 6.18 \\ \bottomrule
   \end{tabular}}
   \caption{Reconstruction performance on CATH4.3 test set. We highlight the best model in color.}
   \label{tab:reconstruction}
\end{table}
